On the Computational Power of Online Gradient Descent

We prove that the evolution of weight vectors in online gradient descent can encode arbitrary polynomial-space computations, even in very simple learning settings. Our results imply that, under weak complexity-theoretic assumptions, it is impossible to reason efficiently about the fine-grained behavior of online gradient descent.

==> tex/older_implementation.tex <==
\section{API}

\begin{table}
\caption{Public API}
\label{tab:public-api}
\centering
\begin{tabular}{@{}lll@{}}
  \toprule
  \textbf{Function} & \textbf{Precondition(s)} & \textbf{Description} \\ \midrule
  % reset(i_1)
  \reset{i_1} &
  $i_1 \in \memory$ &
  $w_{i_1} \leftarrow 0$ \\
  &
  $w_{i_1} \in \binary$ &
  \\ \midrule
  % copy(i_1, i_2)
  \cpy{i_1}{i_2} &
  $i_1, i_2 \in \memory$ &
  $w_{i_2} \leftarrow w_{i_1}$ \\
  &
  $w_{i_1} \in \binary$ &
  \\
  &
  $w_{i_2} = 0$ &
  \\ \midrule
  % destructive_nand(i_1, i_2, i_3)
  \dnand{i_1}{i_2}{i_3} &
  $i_1, i_2, i_3 \in \memory$ &
  $w_{i_3} \leftarrow \text{NAND}(w_{i_1}, w_{i_2})$ \\
  &
  $w_{i_1} \in \binary$ &
  $w_{i_1} \leftarrow 0$ \\
  &
  $w_{i_2} \in \binary$ &
  $w_{i_2} \leftarrow 0$ \\
  &
  $w_{i_3} = 0$ &
  \\ \midrule
  % initialize_true(i_1)
  \inputT{i_1} &
  $i_1 \in \memory$ &
  If $w_{i_1} == 0$, $w_{i_1} \leftarrow +1$ \\
  &
  $w_{i_1} \in \ubinary$ &
  \\ \midrule
  % initialize_false(i_1)
  \inputF{i_1} &
  $i_1 \in \memory$ &
  If $w_{i_1} == 0$, $w_{i_1} \leftarrow -1$ \\
  &
  $w_{i_1} \in \ubinary$ &
  \\
  \bottomrule
\end{tabular}
\end{table}

\begin{lemma}[cf. \cite{APR14}, Lemma 3]
  There is a family of circuits $\C$ of size polynomial in the number of inputs and of polynomial complexity such that \cpath{} is $\PSPACE$-complete.
\end{lemma}

The \sgdsvm{} problem is as follows. % TODO





\begin{figure}

\centering

\begin{subfigure}{.5\textwidth}
  \begin{center}
\centerline{\includegraphics[scale=0.33]{gates1}} 
\caption{The circuit. \label{fig:clusterA}}
\end{center}\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \begin{center}
  \vspace{1cm}
\centerline{\includegraphics[scale=0.45]{gates2}} 
\vspace{0.9cm}
\caption{The weight vector keeps track of the input/output in the circuit gates. \label{fig:clusterA}}
\end{center}\end{subfigure}
\caption{We show that OGD can simulate an arbitrary circuit.}
\label{fig:test}
\end{figure}





\begin{theorem}
  \sgdsvm{} is $\PSPACE$-hard.
\end{theorem}



\begin{proof}
  We prove the theorem by reduction from the \cpath{} problem. Suppose we have an instance of the \cpath{} problem: a circuit $\C$ and a target binary string $t$. We begin by converting $\C$ into an equivalent circuit $\C'$ which only uses NAND gates instead of the standard AND, OR, and NOT gates.
  
  Let $n$ be the number of bits in $t$ and $m$ be the number of gates in $\C'$. We number the input bits from $1$ to $n$. We also fix a topological ordering of the gates of $\C'$ and number them in that order from $n + 1$ to $n + m$. Finally, we reserve $n + m + 1$ and $n + m + 2$ for two special registers.
  
  Our training set uses $d = n + m + 2$ dimensions, corresponding with this numbering. We construct our training set in multiple phases using the API found in Table~\ref{tab:public-api}.
  
  In Phase 1, we iterate through $i = 1, \ldots, n$. In iteration $i$, we add \inputF{i} to the end of our training set.
  
  In Phase 2, we iterate through $i = n + 1, \ldots, n + m$. In iteration $i$, we examine the gate in $\C'$ numbered $i$; suppose its inputs are $i_1$ and $i_2$. We add \cpy{i_1}{n+m+1}, \cpy{i_2}{n+m+2}, \dnand{n+m+1}{n+m+2}{i} to the end of our training set, in that order.
  
  In Phase 3, we iterate through $i = 1, \ldots, n$. In iteration $i$, we examine the $i^{th}$ output gate of $\C'$; suppose it is $i_1$. We add \reset{i} and \cpy{i_1}{i} to the end of our training set, in that order.
  
  In Phase 4, we iterate through $i = n+1, \ldots, n + m$. In iteration $i$, we add \reset{i} to the end of our training set.
  
  % TODO
\end{proof}

\section{API Implementation}

Now that we have described in a high level how to simulate the circuit computation using the Online Gradient Descent updates, we proceed by giving the technical details of the implementation for each ``atomic'' function operation on the circuit bits: $\texttt{add}, \texttt{reset}, \texttt{copy}, \texttt{destructive\_nand}, \texttt{input\_true}, \texttt{input\_false}$. Note that in all of our constructions the training examples required are extremely sparse having $\le3$ non-zero coordinates.


\begin{table}
\caption{Private API}
\label{tab:private-api}
\centering
\begin{tabular}{@{}lll@{}}
  \toprule
  \textbf{Function} & \textbf{Precondition(s)} & \textbf{Description} \\ \midrule
  % add(i_1, c)
  \add{i_1}{c} &
  $i_1 \in \memory$ &
  $w_{i_1} \leftarrow w_{i_1} + c$ \\
  &
  $|c| \le 2$&
  \\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Implementation of \add{i_1}{c}}
For an index $i_1 \in \memory$ and a given constant $|c|\le2$, \add{i_1}{c} has the effect of adding $c$ to the weight coordinate indexed by $i_1$. This is the only operation in our private API and is used in the implementation of all other operations.

How can one add $c$ to a weight coordinate $i_1$? Recall that the only operations performed during OGD are updates based on the gradient of the loss function so we will leverage exactly this. The hinge loss function is:
\[
  L(\vec{w}, \vec{x}, y) = \max \{1 - y \vec{w}\cdot \vec{x}) , 0\}
\]
and the update is:
\[
  \frac{\partial L(\vec{w}, \vec{x}, y)}{\partial w_i}
  =
  \begin{cases}
    -y x_i & \text{if } y \vec{w}\cdot \vec{x} < 1 \\
    0 & \text{if } y \vec{w}\cdot \vec{x} > 1
  \end{cases}
\]

For our reduction, we have the freedom to select the training datapoint $\vec{x}$ along with its label $y$. We pick the $i_1$-th coordinate to be $x_{i_1}=\tfrac{c}{10}$, whereas $x_i=0, \forall i\neq i_1$ and its label to be $y=+1$. After the update the weight $w_{i_1}\leftarrow w_{i_1}-\left(-(+1)(x_{i_1})\right) \implies w_{i_1}\leftarrow w_{i_1}+\tfrac{c}{10}$. The result of the first update can also be seen in the first row of Table~\ref{tab:add}.  Repeating the same training example a constant number of times will result in the desired outcome of adding $c$ to the weight coordinate $i_1$.

\begin{table}
\caption{Training data for \add{i_1}{c}.}
\label{tab:add}
\centering
\begin{tabular}{@{}ccr@{}l@{$) \to ($}l@{)}@{}}
  \toprule
  $x_{i_1}$ & $y$ & \multicolumn{3}{@{}c@{}}{Effect on $(w_{i_1})$} \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1}$ & $w_{i_1} + \frac{1}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{1}{10} c$ & $w_{i_1} + \frac{2}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{2}{10} c$ & $w_{i_1} + \frac{3}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{3}{10} c$ & $w_{i_1} + \frac{4}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{4}{10} c$ & $w_{i_1} + \frac{5}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{5}{10} c$ & $w_{i_1} + \frac{6}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{6}{10} c$ & $w_{i_1} + \frac{7}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{7}{10} c$ & $w_{i_1} + \frac{8}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{8}{10} c$ & $w_{i_1} + \frac{9}{10} c$ \\ \midrule
  $\frac{1}{10} c$ & $+1$ & $($ & $w_{i_1} + \frac{9}{10} c$ & $w_{i_1} + c$ \\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Implementation of \reset{i_1}}
The reset gadget (see~Table~\ref{tab:reset}) takes as input one index $i_1$ and resets the corresponding weight coordinate to 0 independent of what this coordinate used to be (either $-1$ or $+1$). If we knew the value of $w_{i_1}$, things would be straightforward given that we have implemented the $\texttt{add}$ gadget: in the case where $w_{i_1}=+1$ we would just do \add{i_1}{-1} and in the case $w_{i_1}=-1$ we would just do \add{i_1}{+1}.

Now that we don't know $w_{i_1}$, the idea is to first map it to $-1$ and perform \add{i_1}{+1} and finish. What is an appropriate training example that will allow us to map $+1 \rightarrow -1$ and $-1\rightarrow -1$. Let the training example be labeled with $y=+1$ and have $x_{i_1}=-2$ and 0 on the rest of its coordinates.

In the case of $w_{i_1}= -1$, we have $y \vec{w}\cdot \vec{x} > 1$ and so there is no update since the gradient of the hinge loss is 0, hence $w_{i_1}$ remains $-1$. If $w_{i_1}= +1$, we have $y \vec{w}\cdot \vec{x} = (+1)(-2) < 1$, so after the update we get: $w_{i_1}\leftarrow w_{i_1} + (+1)(-2)\implies w_{i_1}\leftarrow -1$, as desired. The final step is to \add{i_1}{+1} and this will make the weight vector's $i_1$-th coordinate 0.


\begin{table}



        \centering
        %\caption{}
        \label{multiprogram}
        \begin{tabular}{c|c|c|c|c|c|c|c|c|}
            \cline{2-8}
             & \multicolumn{7}{|c|}{$\texttt{weights}=(w_1,w_2,w_3,w_4,w_5,w_6,w_7)$}\\
            \cline{2-8}
            \hline
           
             \multicolumn{1}{|c|}{\#$\texttt{iter}$}& $w_1$ & $w_2$ & $w_3$ & $w_4$ & $w_5$ & $w_6$ & $w_7$\\
             \hline
             \multicolumn{1}{|c|}{1} &$\texttt{0}$ & $\texttt{0}$ & $\texttt{0}$ & $\texttt{0}$ &$\texttt{0}$  &$\texttt{0}$  &$\texttt{0}$ \\
            \hline
              \multicolumn{1}{|c|}{2} &\cellcolor{red!25}$\texttt{-1}$ &  $\texttt{0}$ & $\texttt{0}$ & $\texttt{0}$ &$\texttt{0}$  &$\texttt{0}$  &$\texttt{0}$ \\
             \hline
             \multicolumn{1}{|c|}{3} &\cellcolor{red!25}$\texttt{-1}$ &  \cellcolor{red!25}$\texttt{-1}$ & $\texttt{0}$ & $\texttt{0}$ &$\texttt{0}$  &$\texttt{0}$  &$\texttt{0}$ \\
             \hline
              \multicolumn{1}{|c|}{4} &\cellcolor{red!25}$\texttt{-1}$ &  \cellcolor{red!25}$\texttt{-1}$ & \cellcolor{green!25}$\texttt{+1}$ & $\texttt{0}$ &$\texttt{0}$  &$\texttt{0}$  &$\texttt{0}$ \\
             \hline
              \multicolumn{1}{|c|}{5} &\cellcolor{red!25}$\texttt{-1}$ &\cellcolor{red!25}  $\texttt{-1}$ &\cellcolor{green!25} $\texttt{+1}$ &\cellcolor{red!25} $\texttt{-1}$ &$\texttt{0}$  &$\texttt{0}$  &$\texttt{0}$ \\
             \hline
              \multicolumn{1}{|c|}{6} &\cellcolor{red!25}$\texttt{-1}$ &\cellcolor{red!25}  $\texttt{-1}$ &\cellcolor{green!25} $\texttt{+1}$ &\cellcolor{red!25} $\texttt{-1}$ &\cellcolor{green!25}$\texttt{+1}$  &$\texttt{0}$  &$\texttt{0}$ \\
             \hline
               \multicolumn{1}{|c|}{7} &\cellcolor{red!25}$\texttt{-1}$ &\cellcolor{red!25}  $\texttt{-1}$ &\cellcolor{green!25} $\texttt{+1}$ & \cellcolor{red!25}$\texttt{-1}$ &\cellcolor{green!25}$\texttt{+1}$  &\cellcolor{green!25}$\cellcolor{green!25}\texttt{+1}$  &$\texttt{0}$ \\
             \hline
              \multicolumn{1}{|c|}{8} &\cellcolor{red!25}$\texttt{-1}$ &  \cellcolor{red!25}$\texttt{-1}$ &\cellcolor{green!25} $\texttt{+1}$ &\cellcolor{red!25} $\texttt{-1}$ &\cellcolor{green!25}$\texttt{+1}$  &\cellcolor{green!25}$\texttt{+1}$  &\cellcolor{green!25}$\texttt{+1}$ \\
             \hline
            \hline
             \cline{2-8}
             & \multicolumn{7}{|c|}{$\texttt{unset=0, true=+1, false=-1}$}\\
            \cline{2-8}
        \end{tabular}
    \end{table}

\begin{table}
        \centering
        %\caption{}
        \label{multiprogram}
        \begin{tabular}{c|c|c|c|c|c|c|c|c|}
            \cline{2-8}
             & \multicolumn{7}{|c|}{$\texttt{U=unset,T=true, F=false}$}\\
            \cline{2-8}
           % \hline
           
           

        \end{tabular}
    \end{table}




\begin{table}
\caption{Training data for \reset{i_1}.}
\label{tab:reset}
\centering
\begin{tabular}{@{}ccr@{}r@{$) \to ($}r@{)}@{}}
  \toprule
  $x_{i_1}$ & $y$ & \multicolumn{3}{c}{Effect on $(w_{i_1})$} \\ \midrule
  $-2$ & $+1$ & $($ & $-1$ & $-1$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $-1$ \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{+1}} & $($ & $-1$ & $0$ \\
  \multicolumn{2}{c}{} & $($ & $-1$ & $0$ \\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Implementation of \cpy{i_1}{i_2}}
Suppose we want to copy the $i_1$-th coordinate of the weight vector to its $i_2$-th coordinate. How can we do that using only gradient updates? Again the difficulty in performing the copy operation stems from the fact that we don't know the values of the coordinates; if we did know them, for example, if $w_{i_1}=-1$ and $w_{i_2}=1$ in order to perform \cpy{i_1}{i_2}, we could just do \add{i_2}{-2}.

The sequence of operations together with the resulting weight vector after the gradient updates are provided in Table~\ref{tab:cpy}. Observe that in the end, the value of the $i_2$-th coordinate of the weight vector is exactly the same as the $i_1$-coordinate and the operation \cpy{i_1}{i_2} is performed correctly.

We are going to use two training examples. The first training example has label $+1$, $x_{i_1}=-4,x_{i_2}=+2$ and $x_i=0, \forall i\neq i_1,i_2$. The second training example has label $+1$, $x_{i_1}=-4,x_{i_2}=0$ and $x_i=0, \forall i\neq i_1,i_2$. 

\begin{itemize}
\item Let's focus in the case where $w_{i_1}=-1$ (upper half of every row in Table~\ref{tab:cpy}). Without loss of generality let $w_{i_2}=0$ since otherwise we can just perform \reset{i_2} using previously defined gadgets. 

The gradient update on the first example will not affect the weight vector as $y \vec{w}\cdot \vec{x} = (+1)(-1)(-4)= 4> 1$. Then we just add $+2$ to get $(w_{i_1},w_{i_2})=(+1,0)$. The gradient update on the second training example leads to $w_{i_1}\leftarrow w_{i_1}-4\implies w_{i_1}\leftarrow -3$. After the last two addition steps, we end up with the desired $(w_{i_1},w_{i_2})=(-1,-1)$ outcome. 

\item This is similar to the previous case and by tracking down the gradient updates we end up with the desired $(w_{i_1},w_{i_2})=(+1,+1)$ outcome. 

\end{itemize}




\begin{table}
\caption{Training data for \cpy{i_1}{i_2}.}
\label{tab:cpy}
\centering
\begin{tabular}{@{}cccr@{}r@{, }r@{$) \to ($}r@{, }r@{)}@{}}
  \toprule
  $x_{i_1}$ & $x_{i_2}$ & $y$ & \multicolumn{5}{c}{Effect on $(w_{i_1}, w_{i_2})$} \\ \midrule
  $-4$ & $+2$ & $+1$ & $($ & $-1$ & $0$ & $-1$ & $0$ \\
  \multicolumn{3}{c}{} & $($ & $+1$ & $0$ & $-3$ & $+2$ \\ \midrule
  \multicolumn{3}{c}{\add{i_1}{+2}} & $($ & $-1$ & $0$ & $+1$ & $0$ \\
  \multicolumn{3}{c}{} & $($ & $-3$ & $+2$ & $-1$ & $+2$ \\ \midrule
  $-4$ & $0$ & $+1$ & $($ & $+1$ & $0$ & $-3$ & $0$ \\
  \multicolumn{3}{c}{} & $($ & $-1$ & $+2$ & $-1$ & $+2$ \\ \midrule
  \multicolumn{3}{c}{\add{i_1}{+2}} & $($ & $-3$ & $0$ & $-1$ & $0$ \\
  \multicolumn{3}{c}{} & $($ & $-1$ & $+2$ & $+1$ & $+2$ \\ \midrule
  \multicolumn{3}{c}{\add{i_2}{-1}} & $($ & $-1$ & $0$ & $-1$ & $-1$ \\
  \multicolumn{3}{c}{} & $($ & $+1$ & $+2$ & $+1$ & $+1$ \\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Implementation of \dnand{i_1}{i_2}{i_3}}
We want to implement a NAND gate with inputs the coordinates $w_{i_1},w_{i_2}$ and output the result in $w_{i_3}$. Along the process we will zero out the input coordinates that's why we call it destructive NAND. The operations needed are provided in Table~\ref{tab:dnand}. Notice that we should end up with $w_{i_3}=+1$ except for the case when $w_{i_1}=w_{i_2}=+1$ for which it should be $w_{i_3}=-1$.

We focus on the bottom line of each row in Table~\ref{tab:dnand}. The derivation for the other rows is completely similar. The weight vector has $w_{i_1}$, $w_{i_2}$ set and we want to output their NAND in the coordinate $w_{i_3}$. We will implement this in 5 steps. First we add the constant $-1$ to $w_{i_3}$ so that we set to to $-1$.

The next row is the only step that may be a bit unclear and that requires some calculations that are provided here. The training example has label $y=+1$, with $x_{i_1}=x_{i_2}=x_{i_3}=-2$ and $x_{i}=0,\forall i\neq i_1,i_2,i_3$. 

\begin{itemize}
\item If the weights are $(-1,-1,-1)$ then $y \vec{w}\cdot \vec{x}=(+1)(+2+2+2)=6 > 1$ so there is no update in this case.

\item If the weights are $(-1,+1,-1)$ then $y \vec{w}\cdot \vec{x}=(+1)(+2-2+2)=2 > 1$ so there is no update in this case.

\item If the weights are $(+1,-1,-1)$, similarly there is no update.

\item If the weights are $(+1,+1,-1)$, then $y \vec{w}\cdot \vec{x}=(+1)(-2-2+2)=-2 < 1$ so the gradient in this case is $ -y x_i=-(+1)(-2)=+2$ for every coordinate in the weight vector which now becomes $(-1,-1,-3)$ after subtracting the gradient.

\end{itemize}

The next 3 steps are easily interpretable given our previous gadgets.


\begin{table}
\caption{Training data for \dnand{i_1}{i_2}{i_3}.}
\label{tab:dnand}
\centering
\begin{tabular}{@{}ccccr@{}r@{, }r@{, }r@{$) \to ($}r@{, }r@{, }r@{)}@{}}
  \toprule
  $x_{i_1}$ & $x_{i_2}$ & $x_{i_3}$ & $y$ & \multicolumn{7}{c}{Effect on $(w_{i_1}, w_{i_2}, w_{i_3})$} \\ \midrule
  \multicolumn{4}{c}{\add{i_3}{-1}} & $($ & $-1$ & $-1$ & $0$ & $-1$ & $-1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $-1$ & $+1$ & $0$ & $-1$ & $+1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $+1$ & $-1$ & $0$ & $+1$ & $-1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $+1$ & $+1$ & $0$ & $+1$ & $+1$ & $-1$ \\ \midrule
  $-2$ & $-2$ & $-2$ & $+1$ & $($ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $-1$ & $+1$ & $-1$ & $-1$ & $+1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $+1$ & $-1$ & $-1$ & $+1$ & $-1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $+1$ & $+1$ & $-1$ & $-1$ & $-1$ & $-3$ \\ \midrule
  \multicolumn{4}{c}{\reset{i_1}} & $($ & $-1$ & $-1$ & $-1$ & $0$ & $-1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $-1$ & $+1$ & $-1$ & $0$ & $+1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $+1$ & $-1$ & $-1$ & $0$ & $-1$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $-1$ & $-1$ & $-3$ & $0$ & $-1$ & $-3$ \\ \midrule
  \multicolumn{4}{c}{\reset{i_2}} & $($ & $0$ & $-1$ & $-1$ & $0$ & $0$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $0$ & $+1$ & $-1$ & $0$ & $0$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $0$ & $-1$ & $-1$ & $0$ & $0$ & $-1$ \\
  \multicolumn{4}{c}{} & $($ & $0$ & $-1$ & $-3$ & $0$ & $0$ & $-3$ \\ \midrule
  \multicolumn{4}{c}{\add{i_3}{+2}} & $($ & $0$ & $0$ & $-1$ & $0$ & $0$ & $+1$ \\
  \multicolumn{4}{c}{} & $($ & $0$ & $0$ & $-1$ & $0$ & $0$ & $+1$ \\
  \multicolumn{4}{c}{} & $($ & $0$ & $0$ & $-1$ & $0$ & $0$ & $+1$ \\
  \multicolumn{4}{c}{} & $($ & $0$ & $0$ & $-3$ & $0$ & $0$ & $-1$ \\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Implementation for \inputT{i_1}}
The effect of \inputT{i_1} is to map the $i_1$-th coordinate (which is either $-1,0,+1$) to $+1$, unless it is $-1$ in which case it should remain $-1$. The implementation can be found in~Table~\ref{tab:inputT}.

The 4 steps in Table~\ref{tab:inputT} with the \texttt{add} gadgets should be clear by now. Here we give the calculations of the gradients and updates for the 3 steps that contain training examples.

\begin{itemize}
\item The training example has label $y=+1$, with $x_{i_1}=+3$ and $x_{i}=0,\forall i\neq i_1$. If $w_{i_1}=0$ then $y \vec{w}\cdot \vec{x}=(+1)(0)=0 < 1$ so the gradient step will add $yx_{i_1}=(+1)(+3)=3$ to $w_{i_1}$. If $w_{i_1}=+1$ then $y \vec{w}\cdot \vec{x}=(+1)(+1)(+3)=3 > 1$ so there is no update. If $w_{i_1}=+2$, then again there is no update. 

\item The training example has label $y=+1$, with $x_{i_1}=+4$ and $x_{i}=0,\forall i\neq i_1$. If $w_{i_1}=+2$ then $y \vec{w}\cdot \vec{x}=(+1)(+2)(+4)=+8 > 1$ so there is no update. If $w_{i_1}=0$, then $y \vec{w}\cdot \vec{x}=0 < 1$, so the gradient step will add $yx_{i_1}=(+1)(+4)=4$ to $w_{i_1}$. If $w_{i_1}=+1$ then $y \vec{w}\cdot \vec{x}=(+1)(+1)(+4)=4 > 1$ so there is no update. 


\item Training on the final training example is similar to the first case above.

\end{itemize}

\begin{table}
\caption{Training data for \inputT{i_1}.}
\label{tab:inputT}
\centering
\begin{tabular}{@{}ccr@{}r@{$) \to ($}r@{)}@{}}
  \toprule
  $x_{i_1}$ & $y$ & \multicolumn{3}{c}{Effect on $(w_{i_1})$} \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{+1}} & $($ & $-1$ & $0$ \\
  \multicolumn{2}{c}{} & $($ & $0$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $+2$ \\ \midrule
  $+3$ & $+1$ & $($ & $0$ & $+3$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+2$ & $+2$ \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{-1}} & $($ & $+3$ & $+2$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $0$ \\
  \multicolumn{2}{c}{} & $($ & $+2$ & $+1$ \\ \midrule
  $+4$ & $+1$ & $($ & $+2$ & $+2$ \\
  \multicolumn{2}{c}{} & $($ & $0$ & $+4$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $+1$ \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{-1}} & $($ & $+2$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+4$ & $+3$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $0$ \\ \midrule
  $+3$ & $+1$ & $($ & $+1$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+3$ & $+3$ \\
  \multicolumn{2}{c}{} & $($ & $0$ & $+3$ \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{-2}} & $($ & $+1$ & $-1$ \\
  \multicolumn{2}{c}{} & $($ & $+3$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+3$ & $+1$ \\ \midrule
  \bottomrule
\end{tabular}
\end{table}

\subsection{Implementation of \inputF{i_1}}
The effect of \inputF{i_1} is to map the $i_1$-th coordinate (which is either $-1,0,+1$) to $-1$, unless it is $+1$ in which case it should remain $+1$. The implementation can be found in~Table~\ref{tab:inputF} and the calculations can be done similarly to the \inputT{i_1} implementation previously.


\begin{table}
\caption{Training data for \inputF{i_1}.}
\label{tab:inputF}
\centering
\begin{tabular}{@{}ccr@{}r@{$) \to ($}r@{)}@{}}
  \toprule
  $x_{i_1}$ & $y$ & \multicolumn{3}{c}{Effect on $(w_{i_1})$} \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{+1}} & $($ & $-1$ & $0$ \\
  \multicolumn{2}{c}{} & $($ & $0$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $+2$ \\ \midrule
  $+3$ & $+1$ & $($ & $0$ & $+3$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+2$ & $+2$ \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{-1}} & $($ & $+3$ & $+2$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $0$ \\
  \multicolumn{2}{c}{} & $($ & $+2$ & $+1$ \\ \midrule
  $+2$ & $+1$ & $($ & $+2$ & $+2$ \\
  \multicolumn{2}{c}{} & $($ & $0$ & $+2$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $+1$ \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{-1}} & $($ & $+2$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+2$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $0$ \\ \midrule
  $+3$ & $+1$ & $($ & $+1$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $+1$ \\
  \multicolumn{2}{c}{} & $($ & $0$ & $+3$ \\ \midrule
  \multicolumn{2}{c}{\add{i_1}{-2}} & $($ & $+1$ & $-1$ \\
  \multicolumn{2}{c}{} & $($ & $+1$ & $-1$ \\
  \multicolumn{2}{c}{} & $($ & $+3$ & $+1$ \\ \midrule
  \bottomrule
\end{tabular}
\end{table}

\subsection{Handling the Bias Term}

\ifx\undefined\mainfile

\end{document}

\fi
